On The Synergy Between Ariel And Ground-Based High-Resolution Spectroscopy

Since the first discovery of an extra-solar planet around a main-sequence star, in 1995, the number of detected exoplanets has increased enormously. Over the past two decades, observational instruments (both onboard and on ground-based facilities) have revealed an astonishing diversity in planetary physical features (i. e. mass and radius), and orbital parameters (e.g. period, semi-major axis, inclination). Exoplanetary atmospheres provide direct clues to understand the origin of these differences through their observable spectral imprints. In the near future, upcoming ground and space-based telescopes will shift the focus of exoplanetary science from an era of 'species discovery' to one of 'atmospheric characterization'. In this context, the Atmospheric Remote-sensing Infrared Exoplanet Large (Ariel) survey, will play a key role. As it is designed to observe and characterize a large and diverse sample of exoplanets, Ariel will provide constraints on a wide gamut of atmospheric properties allowing us to extract much more information than has been possible so far (e.g. insights into the planetary formation and evolution processes). The low resolution spectra obtained with Ariel will probe layers different from those observed by ground-based high resolution spectroscopy, therefore the synergy between these two techniques offers a unique opportunity to understanding the physics of planetary atmospheres. In this paper, we set the basis for building up a framework to effectively utilise, at near-infrared wavelengths, high-resolution datasets (analyzed via the cross-correlation technique) with spectral retrieval analyses based on Ariel low-resolution spectroscopy. We show preliminary results, using a benchmark object, namely HD 209458 b, addressing the possibility of providing improved constraints on the temperature structure and molecular/atomic abundances.

==> abbr.tex <==
@String { \aap      = "Astronomy and Astrophysics" }
@String { \aj       = "Astronomical Journal" }
@String { \apj      = "Astrophysical Journal" }
@String { \apjl     = "Astrophysical Journal, Letters" }
@String { \apjs     = "Astrophysical Journal, Supplement“ }
@String { \apss     = "Astrophysics and Space Science“ }
@String { \araa     = “Annual Review of Astron and Astrophys" }
@String { \hm       = "Historia Mathematica" }
@String { \icarus   = "Icarus" }
@String { \jqsrt   = "Journal of Quantitiative Spectroscopy and Radiative Transfer" }
@String {\mnras     = "Monthly Notices of the RAS"}
@String { \nat      = "Nature" }
@String {\pasp = "Publications of the ASP" }
@String { \ssr      = "Space Science Reviews" }
